Differentiable Surface Triangulation

Triangle meshes remain the most popular data representation for surface geometry. This ubiquitous representation is essentially a hybrid one that decouples continuous vertex locations from the discrete topological triangulation. Unfortunately, the combinatorial nature of the triangulation prevents taking derivatives over the space of possible meshings of any given surface. As a result, to date, mesh processing and optimization techniques have been unable to truly take advantage of modular gradient descent components of modern optimization frameworks. In this work, we present a differentiable surface triangulation that enables optimization for any per-vertex or per-face differentiable objective function over the space of underlying surface triangulations. Our method builds on the result that any 2D triangulation can be achieved by a suitably perturbed weighted Delaunay triangulation. We translate this result into a computational algorithm by proposing a soft relaxation of the classical weighted Delaunay triangulation and optimizing over vertex weights and vertex locations. We extend the algorithm to 3D by decomposing shapes into developable sets and differentiably meshing each set with suitable boundary constraints. We demonstrate the efficacy of our method on various planar and surface meshes on a range of difficult-to-optimize objective functions. Our code can be found online: https://github.com/mrakotosaon/diff-surface-triangulation.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.79.  Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

==> sections/method_backup.tex <==
\section{Method}
Let $(V', T)$ represent a triangulation of a surface in 3D space, with $V' = (v'_1, \dots, v'_n), v'_i \in \mathbb{R}^3$ vertices, and $T$ its triangular faces. A common strategy for triangulating a manifold surface is to first find a 2D parameterization that maps the surface to a planar 2D domain,  then sample a set of vertices $V = (v_1, \dots, v_n), v_i \in \mathbb{R}^2$ in the 2D domain, and compute a triangulation which respects the chosen vertices. Our method relies on the ubiquitous Delaunay triangulation~\cite{book:DT_2016} ($\dt$), used for triangulating a given 2D vertex set. We denote it as $T = \dt(V)$. A Delaunay triangulation always includes all chosen vertices, and is, uniquely defined with respect to them, as long as the points are in general position. In order to gain more control over the triangulation,  one can consider a \emph{weighted} Delaunay triangulation~\cite{toth2017handbook} $T = \wdt(V, W)$, where each vertex $v_i$ has a scalar weight $w_i$, with $W=(w_1, \dots, w_n)$. Traditional methods for computing a $\wdt$ are typically not differentiable, as the space of all possible faces is combinatorial.


We propose a differentiable weighted Delaunay triangulation $\dwdt(V, W)$ that is differentiable with respect to both the vertex positions $V$ and the weights $W$. In conjunction with a parameterization $m$ that defines a bijective and piecewise differentiable mapping $m$ from a surface in 3D to a 2D parameter space, $\dwdt$ enables a differentiable pipeline for triangulating 3D domains. We describe our differentiable triangulation approach in two parts (see Figure~\ref{fig:overview}). First, in Section~\ref{sec:diff_2d_meshing}, we describe the differentiable weighted 2D Delaunay triangulation $\dwdt$. In this part, we first focus on the definition of $\dt$ and the existence of triangles, w.r.t. vertex positions and weights, and then replace the  binary  triangle existence function with a smooth existence \emph{probability}, again defined w.r.t the vertex positions and weights, in a way that naturally follows from the definition of $\dt$. This yields a \emph{soft} and differentiable notion of a triangulation that can easily be generalized to a weighted Delaunay triangulation. Then, in Section~\ref{sec:3d_param}, we describe a parameterization $m$ that maps between a manifold surface and our 2D Delaunay triangulation to obtain $\dwdt$ on 3D surfaces, before describing the losses and optimization setup in Section~\ref{sec:losses}.

%A given set of vertices generally admits many different manifold and non-manifold triangulations. A common strategy to obtain a manifold triangulation from a set of vertices is to define an operator on the set of vertices that returns a triangulation, such as the Delaunay Triangulation~\cite{} $F = \mathcal{D}(V)$. To obtain more control over the triangulation, the vertices can be augmented with additional properties, such as weights in the weighted Delaunay Triangulation~\cite{} $F = \mathcal{T}(V, W)$. This operator is typically not differentiable with respect to its inputs.

%\subsection{Overview}

\subsection{Differentiable Weighted Delaunay Triangulation}
\label{sec:diff_2d_meshing}

Assume we are given a set of vertices $V=\{v_1,...,v_{|V|}\}$ with $v_j \in\mathbb{R}^2$. Consider the set of all possible triangles defined over these vertices, i.e., all possible triplets of vertices:
\begin{equation}
    T^* = \left\{\left(v_j,v_k,v_l\right) | v_j,v_k,v_l\in V \right\}.
\end{equation}
Any triangulation of the vertices $V$ is a subset of all possible triangles $T\subset T^*$ on $V$, and we can consider the triangulation's \emph{existence} function $e:T^* \to \left\{0,1\right\}$, defined for any triplet  $t_i\in T^*$ as
\begin{equation}
\label{eq:existence}
    e_i = \begin{cases}
      1 &t \in T\\
      0 &t \notin T.
    \end{cases}
\end{equation}
From this perspective, the binary and discrete existence function is the cause of the combinatorial nature of the triangulation problem. Hence, our main goal is to define a \emph{smooth} formulation in which this function is differentiable as to enable gradient-based optimization.
%
We achieve this by extending $\wdt$ to the smooth setting.



Towards gaining intuition into $\wdt$, let us first consider the classic, non-weighted \emph{Delaunay triangulation} $\dt(V)$ of a given set of vertices $V$. This triangulation is defined by considering each possible triangle $t \in T^*$ and deeming it as part of the triangulation $\dt(V)$ if and only if its circumcenter is the shared vertex of the three Voronoi cells centered at the triangle's vertices (see Figure~\ref{fig:voronoi} for an illustration). The Voronoi cell of vertex $v_j$ is defined as the set of points in $\mathbb{R}^2$ closer to $v_j$ than to any other vertex $v_k\in V$.

Said differently, each pair of vertices $(v_j, v_k)$ divides the 2D plane into two half-spaces: the set of points closer to $v_j$, denoted as $H_{j<k}$, and the set of points closer to $v_k$, denoted as $H_{k<j}$. The Voronoi cell $a_j$ centered at $v_j$ is defined as the intersection of half-spaces $a_j \coloneq \bigcap_{k\neq j} H_{j<k}$. The triangle circumcenter is the intersection point of the three half-space boundaries between the three vertex pairs that define its edges. Hence, we can define the existence function of the Delaunay triangulation for a triplet of vertices, $t_i = (v_j,v_k,v_l)$ with circumcenter $c_i$ as
\begin{equation}
\label{eq:hp_existence}
    e_i = \begin{cases}
      1 & \text{if}\ \ c_i = a_j \cap a_k \cap a_l \\
      0 & \text{otherwise}.
    \end{cases}
\end{equation}
% H_{u<s}, \forall s\neq u, u \in\left\{j,k,l\right\}\\

In a \emph{weighted Delaunay triangulation} ($\wdt$), weights are associated to each vertex, which allows shifting the boundary between the two half-spaces $H_{j<k}$ and $H_{k<j}$, by the relative weights $w_j$ and $w_k$ of the two vertices. The weighted half space $H_{j<k}$ is defined as the set of points $x\in\mathbb{R}^2$ where
\begin{equation}
\label{eq:power_dist}
     \|x - v_j\|_2^2 - w_j^2 \leq \|x - v_k\|_2^2 - w_k^2
    %  2x(v_k-v_j)+(v_j^2 - w_j^2)-(v_k^2 - w_k^2)
    %  \leq 0,
\end{equation}
so that a larger weight pushes the boundary away from the vertex. This
%extends the notion of a
%Voronoi cell: the set of points on which Equation  \eqref{eq:power_dist} is negative are defined as points closer to $v_j$ than $v_k$
allows generalizing the definition of the Voronoi cell to a weighted Voronoi cell. As a result, the existence function Equation \eqref{eq:hp_existence} can be used as-is, with the modified definition of the half-planes, and considering the \emph{weighted} circumcenter of the triangle.
% \begin{equation}
%     c_i = \frac{1}{3}\sum_{j\in t_i} w_j v_j.
% \end{equation}

Thus, weights enable further control over the resulting triangulation, by enabling modifying the Voronoi cells (and therefore, the triangulation itself). In fact, note that it is even possible for a vertex to be excluded from a $\wdt$ (i.e., not be part of any triangle), if the weight difference to any other vertex is so large that the boundary line between the two half-spaces shifts past one of the vertices - a property not possible with classical Delaunay triangulation. We will make use of this property to allow our method to ignore vertices deemed unnecessary, hence producing meshes with a reduced number of vertices. In the following, we consider the weighted triangle circumcenters, denoted by $c_i$, and the weighted Voronoi cells, denoted by $a_i$.

%In that case both vertices are contained within one of the half-space, the other half-space disappears, and the vertex is no longer part of the $\wdt$. We will make use of this
%the same is true, if we consider the weighted Voronoi cells and a weighted version of the triangle circumcenter.


\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{images/voronoi.pdf}
    \caption{\textbf{Triangle probability and reduced Voronoi cell.} A reduced Voronoi cell for a given triangle $t_i$ at a vertex $v_j$ is constructed from the point set that excludes the two other vertices of the triangle. A triangle $t_i$ exists in the Delaunay triangulation, as long as its circumcenter $c_i$ remains inside the reduced Voronoi cell. We base triangle probabilities $p_{i|j}$ on the signed distance from $c_i$ to the boundary of the reduced Voronoi cell.}
    \label{fig:voronoi}
\end{figure}



\paragraph{Parameterizing Triangle Existence with respect to $V,W$. }
%Since we are aiming for a differentiable triangulation operation,
We are interested in how the triangulation $T$ changes as the vertex positions and weights are changed - namely, we aim to analyze the range of vertex positions and weights that do not change its membership function $e_i$ of a triangle $t_i$.

For any triangle $t_i = \left(v_j,v_k,v_l\right)$, we consider the three \emph{reduced} Voronoi cells $a_{j|i}$, $a_{k|i}$, $a_{l|i}$ respectively around the triangle's vertices $v_j$, $v_k$, $v_l$, where we define a reduced Voronoi cell $a_{j|i}$ centered at the triangle vertex $v_j$ as the Voronoi cell created by ignoring the two other vertices of the triangle, $v_k$ and $v_l$ (see Figure~\ref{fig:voronoi}). The triangle $t_i$ is part of the triangulation $T$ as long is its circumcenter $c_i$ remains inside the reduced Voronoi cells around its vertices. Similarly,  $t_i$ is not part of  $T$ as long as its circumcenter remains outside its three reduced Voronoi cells. Note that, by construction, the circumcenter simultaneously enters or exits the three reduced Voronoi cells.
%Therefore, we are going to focus our discussion on a single Voronoi cell $a_{j|i}$ of a triangle $t_i$, but the same applies to all three Voronoi cells.

\paragraph{Continuous Triangle Membership Probabilities}
We now turn to making $\wdt$ differentiable by \emph{relaxing} the binary existence function $e_i$ defined in Equation \eqref{eq:hp_existence} into a continuous  probability function, $p_i$, denoting the probability a triangle $t_i \in T^*$ to exist as a member of the triangulation $T$, defined with respect to vertex positions and weights. The probabilities are based on the signed distance of the triangle circumcenter to the boundary of the reduced Voronoi cells at the triangle vertices: considering a single vertex $v_j$ of the triangle $t_i$, and its reduced Voronoi cell $a_{j|i}$, the probability is defined as:
\begin{equation}
    p_{i|j} := \sigma\big(\alpha\ d(c_i, a_{j|i}) \big),
\end{equation}
%\paul{TODO: aggregation over the 3 Voronoi cells of the triangle}
where $d$ is the signed distance (positive inside, negative outside) from a point $c_i$ to the boundary of a reduced Voronoi cell $a_{j|i}$, and $\alpha$ is a scaling factor for the width of the Sigmoid $\sigma$ (we use $\alpha = 500$ in all experiments).
The Sigmoid gives a smooth transition from a probability close to $1$ inside the reduced Voronoi cell to a probability close to $0$ outside, with a probability $0.5$ if the circumcenter lies on the boundary of the reduced Voronoi cell, i.e., exactly when the discrete triangle membership changes.  %The membership probability of a triangle is then defined as the average over the three probabilities at its vertices $v_j$, $v_k$, and $v_l$:
%\begin{equation}
%    p_i = \frac{1}{3} (p_{j|i} + p_{k|i} + p_{l|i}).
%\end{equation}
Note that since the circumcenter simultaneously enters/exits the reduced Voronoi cells around each vertex, all three probabilities equal $0.5$ at a discrete membership transition.

For each triangle $t_i$, we store the three probabilities $p_{i|j}$, $p_{i|k}$ and $p_{i|l}$ defined for its three vertices, yielding a \emph{soft} 2D triangulation $(V, P)$ with triangle probabilities $P$. Note that we could average the three probabilities $p_{i|*}$ to get a single probability per triangle, however, we found it more convenient to save one probability per triangle vertex, since most losses that we use are defined on vertices. We can, subsequently, convert this mesh into a discrete 2D mesh $(V, T)$, by selecting all triangles where all probabilities are $> 0.5$.
\niloy{consider defining the triangle probability as a symbol, it maybe useful for some other custom objective function}
Recall that all three probabilities $p_{i|*}$ transition above/below $0.5$ at the same time.
%\maks{Do \textit{all three} probabilities have to be $>0.5$? In practice do we take the min of the three?}
This gives us the same results as the discrete $\wdt$, the final triangulation is guaranteed to be manifold.

Since the number of all possible triangles $T^*$ grows cubically with the vertex count, we reduce the number of triangles under consideration by observing that vertices in the triangles of a Delaunay triangulation are typically within the $k$-nearest neighbors of each other, for some small $k$ (we use $k=80$ in all experiments). Thus, at each Voronoi cell $a_j$, we only consider triangles that are within the $k$-nearest neighbors of $v_j$ and set all other triangle probabilities $p_{j|i}$ implicitly to $0$.
\niloy{shall we leave out the symbol as this is ruling out triangles; we can also define $p_i$ to be triangle probability instead of not doing it (earlier in this section)}
Note that since the 2D vertices $V$ change positions during optimization, we recompute nearest neighbours after each iteration of our algorithm.

% For each points:
% \begin{itemize}
%     \item  Compute $k$  nearest neighbours of $p_i$: $N(i)$
%     \item Compute $k$ weighted half planes between $p_i$ and the neighbors $N(i)$: $\{s_{j}\}_{j \in [1, k]}$ as in the equation of page 4 here: https://team.inria.fr/geometrica/files/2015/11/3-weightedDT.pdf
%     \item Compute $k^2$ intersection points between half planes: $\{a_{lm}\}_{(l,m) \in [1, k] \times [1, k]}$
%     \item Compute the minimum signed distance ($d_{lm}$) between each intersection point ($\{a_{lm}\}$) and all half planes except the half planes from the current intersection point ($\{s_{j}\} \backslash \{s_l, s_m\}$) . Each intersection  point corresponds to a potential triangle. The signed distance is negative outside the voronoi cell, positive inside. $d_{lm}$ correspond to the signed distance of the intersection point to the voronoi cell if the two points are not considered.
%     \item The triangle probability is given by:
%     $P(T_{ilm}) = sigmoid(\beta * d_{lm})$
% \end{itemize}


\subsection{3D Surface Parameterization}
\label{sec:3d_param}
So far we have defined differentiable triangulations of 2D sets of vertices. In order to
 apply our $\dwdt$
%to weighted vertices $(V,W)$
on a 3D surface $\mathcal{M}$, we reduce the problem to a set of 2D (triangulation) problems.

First, we construct a bijective piecewise differentiable mapping $m$ between the manifold and the 2D plane, i.e., a 2D parameterization. Next, we elaborate on the computation of this parameterization. %The manifold is defined by an initial 3D mesh $M = (V,W,T)$ with weighted vertices that we aim to optimize.
As a pre-process, since we are not concerened with the original triangulation but only the underlying surface it represents, we initially remesh input models using isotropic explicit remeshing~\cite{cignoni2008meshlab} to yield meshes constituting between $3-5$K triangles. We then decompose the manifold into a set of separate patches $\{\mathcal{P}_1, \mathcal{P}_2, \dots\}$ that can be individually parameterized with less distortion than the whole shape. Individual patches are found with a spectral clustering approach~\cite{ng2002spectral}, using the adjacency matrix for affinity. We used $10$ patches in all experiments.
%
\niloy{this is repeated later?}
Patches that are not homeomorphic to a disc (i.e., multiple separate boundaries) are cut along the shortest geodesic between any two separate boundaries, until only a single boundary remains.

Then, we construct a low-distortion mapping $m$ between the surface of a patch $\mathcal{P}_i$ and the 2D plane using Least-Squares Conformal Maps~\cite{Levy2002LSCM} (LSCM). To lower the distortion of the mapping for patches that are far from developable, we measure the distortion of the mapping as the deviation of the local scale factor from the global average.
\niloy{repeated here: we can keep this vrsion and remove the earlier one}
Patches with high distortion are cut along the shortest geodesic between the area of maximum distortion and any existing boundary. This process is repeated until the maximum distortion of all patches, measured as the ratio between local scale and global average is above $15\%$ and the mapping is bijective. %did not encounter any non-bijective cases when applied to our parts.
We compute this mapping once, as a preprocess, and reuse it in all steps of the optimization.
% \begin{itemize}
%     \item This parametrization can lead to great distortions especially for patches with convex (ear of bunny) area. We cut these patches along a geodesic between the most distorted area and the boundary
%     \item To get a parametrization with the less distortion we cut the patches so that they are homeomorphic to disks. For each couple of non connected boundaries, we iteratively  cut the patches along the shortest geodesic between vertices of the boundaries.
% \end{itemize}
%Given this mapping, we can find the 3D location of
%Thus, our full differentiable triangulation of a 3D surface part is defined as:
%\begin{equation}
%     T' = \wdt\big(\{m(v_i)\ |\ v_i \in V\}, W\big),
% \end{equation}
%which is differentiable w.r.t. the vertex positions $V$ on the 3D part's surface, and their weights $W$.

\paragraph{Differentiable 3D Surface Triangulation}
Given the mapping $m$, we can pull back the computed 2D triangulation $(V, T)$ to a part of the 3D surface $\mathcal{P}_i$ using the inverse mapping $m^{-1}$.
%$M = \big(\{m^{-1}(v_i)\ |\ v_i \in V\}, T\big)$.
%The 3D mesh remains differentiable w.r.t. the 2D vertices $V$
Thus, our differentiable triangulation of a 3D surface patch is defined as:
\begin{equation}
(V', P) := \big(\big(m^{-1}(v_1), \dots, m^{-1}(v_n)\big),\ \dwdt(V, W)\big),
\end{equation}
which gives us the soft 3D triangulation $(V', P)$ that consists of a set of 3D vertices $V'$ and triangle probabilities $P$. Note the probabilities are still controlled by the position of the 2D vertices $V$ and their weights $W$, and that we can obtain a manifold discrete mesh at any time by selecting all triangles where all probabilities $> 0.5$.
Since the mapping $m$ is piecewise differentiable, any loss $\mathcal{L}$ can be applied directly to the 3D vertices $V'$ and triangle probabilities $P$, allowing gradients to propagate back to the parameters $V$ and $W$ that define $V'$ and $P$.
%
%3D mesh $M$. Recall that $\dwdt$ outputs membership probabilities $P$ for triangles in $T^*$ instead of a discrete subset $T \in T^*$. Any differentiable loss can be applied to these probabilities, allowing gradients to propagate back to the parameters $V$ and $W$ that define the probabilities.
%
We discuss the losses we use in our experiments in Section~\ref{sec:losses}.
%a loss $\mathcal{L}$ can be computed directly on the 3D mesh. Thus the
%compute a loss $\mathcal{L}$ directly on the 3D mesh by mapping the computed triangulation back to the 3D surface:
% \begin{equation}
%     \mathcal{L}(M') = \wdt\big(V , W\big).
% \end{equation}

\paragraph{Boundary preservation}
Special care must be taken to preserve the boundary of each patch, so that putting the patches back together does not result in gaps or overlaps. We use a two-part strategy to ensure pieces fit back together. First, we define a loss that repels vertices from the boundary of a patch, which we describe in Section~\ref{sec:losses}. Second, we perform a post-processing step that cuts the 2D mesh $(V, P)$ along the 2D boundary, cutting individual triangles if necessary.

%first decomposing it into parts, and then finding a parameterization of each part that defines a mapping between the part's surface and the 2D plane. The $\dwdt$ can then be applied to the part's surface in three steps. First, we map the part to the 2D plane using the parameterization. Second, we compute the differentiable $\dwdt$ in the plane; and third, we map the triangulation back to the 3D part, where we can compute the loss. We use a parameterization that results in a bijective mapping  that is (piecewise) differentiable, allowing us to

%The vertices $V$ of a 3D part can then be mapped to the 2D plane, where we can apply our differentiable $\dwdt$, before mapping the triangulation back to the 3D part to compute the loss.

% The $\dwdt$ can then be performed in the plane and mapped back to the
% \label{sec:3d_param}
% \begin{itemize}
%     \item We separate a mesh into patches using spectral clustering
%     \item each patch is flattened using LSCM parametrization
%     \item we can translate 2D coordinates to 3D using barycentric position on the fixed original mesh
% \end{itemize}

\subsection{Losses and Optimization}
\label{sec:losses}
Our differentiable triangulation allows us to optimize a triangular mesh on a surface in 3D using any differentiable loss defined on the 3D vertex positions $V$ and triangle probabilities $P$. We experiment with several different losses, combinations of which are useful for both traditional applications, as well as novel ones, as we experimentally show in Section~\ref{sec:results}.


The \emph{triangle size loss} $\mathcal{L}_s$ encourages triangles to have a specified area:
\begin{equation}
    \mathcal{L}_s(V', P) := \frac{1}{\sum_{i,j} p_{i|j}} \sum_{i,j} p_{i|j}\ \left(0.5\ \|(v'_k-v'_j) \times (v'_l-v'_j)\|_2 - A_j \right)^2,
\end{equation}
where $v'_j$, $v'_k$, and $v'_l$ are the 3D vertices of triangle $t_i$, and $A_j$ is the target area at vertex $v_j$.
\noam{why? what does area have to do with number of vertices?} Since the $\wdt$ gives us control over the final number of vertices in a triangulation, this loss allows us, for example, to coarsen a triangulation, when used in conjunction with other losses.

% The \emph{normal error} $\mathcal{L}_n$ encourages alignment of face normals with the normals of the part $\mathcal{P}$:
% \begin{equation}
%     \mathcal{L}_n(V', P, \mathcal{P}) = -\frac{1}{\sum_i p_i} \sum_i p_i\ n_i \frac{1}{3}\left(n^{\mathcal{P}}_j+n^{\mathcal{P}}_k+n^{\mathcal{P}}_l\right),
% \end{equation}
%  where $v'_j$, $v'_k$, and $v'_l$ are the 3D vertices of triangle $t_i$, $n_i$ is its normal, and $n^{\mathcal{P}}_j$ is the normal of $\mathcal{P}$ at vertex $v'_j$.

The \emph{boundary repulsion loss} $\mathcal{L}_b$ encourages vertices to stay inside the 2D boundary of the patch $\mathcal{P}$ during the optimization:
%\begin{equation}
%    \mathcal{L}_b(V, \mathcal{P}) = \frac{1}{|V|} \sum_j 1 - %e^{\epsilon - \min\left(\epsilon,\ (v_j - b_j) n^b_j\right)},
%\end{equation}
%
\begin{equation}
    \mathcal{L}_b(V, \mathcal{P}) := \frac{1}{|V|} \sum_j  e^{\epsilon - \min\left(\epsilon,\ (v_j - b_j) n^b_j\right)}, % -1,
\end{equation}
where $b_j$ is the point on the boundary closest to the vertex $v_j$ and $n^b_j$ is the 2D boundary normal at that point (pointing inward). The repulsion loss is non-zero below a (signed) distance $\epsilon$ from the boundary. We set $\epsilon$ to 0.01 in our experiments. Note that we do not use our probabilities in this loss, since we want all vertices to remain inside the boundary, irrespective of probabilities.

The \emph{angle loss} $\mathcal{L}_a$ encourages triangles to be equilateral.
%
%\begin{align}
%\mathcal{L}_a(V', P, \mathcal{P}) = \frac{1}{\sum_i p_{i|j}} \sum_i p_{i|j} \Big(&\ | \cos(\angle_i^1) - \cos(\frac{\pi}{3}) | \nonumber\\
%     +&\ | \cos(\angle_i^2) - \cos(\frac{\pi}{3}) | \nonumber\\
%     +&\ | \cos(\angle_i^3) - \cos(\frac{\pi}{3}) |\Big),
%\end{align}
%
\begin{align}
\mathcal{L}_a(V', P, \mathcal{P}) := \frac{1}{\sum_{i,j} p_{i|j}} \sum_{i,j} p_{i|j} \ \left| \cos(\angle_j) - \cos({\pi}/{3}) \right|,
\end{align}
where $\angle_j$ is the corner angle of triangle $t_i$ including vertex $v_j$. Note that this loss can be modified to produce isosceles triangles.%, ordered by size (from small to large).
%
%The \emph{angle loss} $\mathcal{L}_a$ encourages triangles to be isosceles with a smaller angle value $a$.
% \begin{align}
%     % \mathcal{L}_a(V', P, \mathcal{P}) = \frac{1}{\sum_i p_i} \sum_i p_i \Delta_a,\ \text{with} \nonumber\\
%     % \Delta_a &= | \cos(\angle_i^1) - \cos(a) | + | \cos(\angle_i^2) - \cos(a) | + | \cos(\angle_i^3) - \cos(\pi-2a) |,
% \mathcal{L}_a(V', P, \mathcal{P}) = \frac{1}{\sum_i p_i} \sum_i p_i \Big(&\ | \cos(\angle_i^1) - \cos(a) | \nonumber\\
%      +&\ | \cos(\angle_i^2) - \cos(a) | \nonumber\\
%      +&\ | \cos(\angle_i^3) - \cos(\pi-2a) |\Big),
%     % | \|(v'_{\sigma(k)}-v'_{\sigma(j)}) \cdot (v'_{\sigma(l)}-v'_{\sigma(j)})\| - cos(a) | +
%     % \| \|(v'_{\sigma(l)}-v'_{\sigma(k)}) \cdot (v'_{\sigma(j)}-v'_{\sigma(k)})\| - cos(a) \| +
%     % \| \|(v'_{\sigma(k)}-v'_{\sigma(l)}) \cdot (v'_{\sigma(j)}-v'_{\sigma(l}))\| - cos(\pi - 2a) \|,
% \end{align}
% where $\angle_i^j$ are the corner angles of triangle $t_i$, ordered by size (from small to large).

The \emph{curvature alignment loss} $\mathcal{L}_c$ encourages two edges per vertex to align to the two directions of the maximum principal curvature vector field $C$. We define it as,
%
%
\begin{align}
\mathcal{L}_c(V', P, \mathcal{P}, C) :=& \frac{-1}{\sum_{i,j} p_{i|j}} \sum_j
    \Big( \nonumber\\
    & \text{LSE}(\cup_{i \in \mathcal{N}_j}\{C_j \cdot e_{jk}\ p_{i|j}, C_j \cdot e_{jl}\ p_{i|j} \}) \nonumber\\
    +\ & \text{LSE}(\cup_{i \in \mathcal{N}_j}\{-C_j \cdot e_{jk}\ p_{i|j}, -C_j \cdot e_{jl}\ p_{i|j} \}) \Big) \nonumber\\
    \text{with } e_{jm} =& (v'_j-v'_m)/{\|v'_j-v'_m \|_2},
\end{align}
%
where $\mathcal{N}_j$ are the triangles adjacent to $v'_j$,  $v'_j$, $v'_k$, $v'_l$ are the 3D vertices of triangle $t_i$, and LSE denotes smooth maximum function LogSumExp over the weighted alignment scores of all edges adjacent to vertex $v'_j$, where each triangle contributes two edges corresponding to $e_{jk}$ and $e_{jl}$. Intuitively, we want to maximize the alignment of the best-aligned edge in a star of each vertex, for both the positive and negative target guidance direction $C_j$.

\paragraph{Optimization}

Given a loss $\mathcal{L}$, as a sum of a selection of the terms above,  we optimize the 3D mesh $M$, parameterized by the 2D vertex positions $V$ and vertex weights $W$. Since our framework is completely differentiable, we use the Adam~\cite{DBLP:journals/corr/KingmaB14} optimizer.  We initialize all vertex weights with random values  and use the mapping of the input mesh vertices to 2D as the initial vertex positions. When triangulating, we instead obtain initial vertex positions by projecting the existing 3D mesh vertices to 2D using the mapping $m$.
%
We use a learning rate of $0.0001$ in all experiments. Please refer to the supplementary video for evolving triangulations over optimization iterations.

